A Fusion-Denoising Attack on InstaHide with Data Augmentation

InstaHide is a state-of-the-art mechanism for protecting private training images, by mixing multiple private images and modifying them such that their visual features are indistinguishable to the naked eye. In recent work, however, Carlini et al. show that it is possible to reconstruct private images from the encrypted dataset generated by InstaHide. Nevertheless, we demonstrate that Carlini et al.'s attack can be easily defeated by incorporating data augmentation into InstaHide. This leads to a natural question: is InstaHide with data augmentation secure? In this paper, we provide a negative answer to this question, by devising an attack for recovering private images from the outputs of InstaHide even when data augmentation is present. The basic idea is to use a comparative network to identify encrypted images that are likely to correspond to the same private image, and then employ a fusion-denoising network for restoring the private image from the encrypted ones, taking into account the effects of data augmentation. Extensive experiments demonstrate the effectiveness of the proposed attack in comparison to Carlini et al.'s attack.

==> tex/sec-defense.tex <==
\section{Defenses}\label{sec-defense}
The experiments demonstrate that 
% \scheme\ can effectively restore private images from the encryption datasets generated by InstaHide with data augmentation. The restored images are still distinguishable even under $|M|=10$ or $\epsilon=0.5$. But 
with the decrease of $|M|$ or the increase of $\epsilon$, the adversary extracts less useful information of the private images.
% , and the visual features of the restored images becomes more obscure. 
In addition, the visual features of the public images mixed in an encryption may impact the corruptness levels of the private images, since relatively flat public images may not effectively corrupt the structures of the private images.
We thus propose two defenses against the proposed attack in this section.
% , i.e., reducing the mixed times of a private image meanwhile increasing the augmentation levels, and increasing the complexity of the visual features of the mixed public images.

\noindent\textbf{Reducing the mixed times of a private image.}
Since \scheme\ can restore distinguishable images even under $|M|=10$, we further reduce the mixed times of a private image to $|M|=2$, 4, 6, 8, and test the performance of \scheme\ and \cite{carlini2020attack} based on parameters $\mathcal{X}_p=\text{CIFAR10}$, $\mathcal{X}_t=\text{CIFAR100}$, $\epsilon_p=\epsilon_t=0.3$. 
%
% Note that in the original InstaHide scheme, $|M|$ typically equals to the number of training epochs, i.e. $|M|$ is generally dozens or hundreds. Therefore, the test cases in this experiment are fairly extreme compared to the real world applications. 
%
Fig.~\ref{fig-defenseM} and \ref{fig-defenseM-exp} show the attack performance and some examples of the restored images, respectively. From Fig.~\ref{fig-defenseM} we see that \scheme\ performs far better than \cite{carlini2020attack} under $|M|_p<10$. This is because the visual features of private images are mainly corrupted by the noise components. \scheme\ can learn the distribution of noise and effectively remove it, whereas \cite{carlini2020attack} could be easily impacted by the salient noise in some severely corrupted encryptions. 
%
Fig.~\ref{fig-defenseM-exp} shows \scheme\ can restore the general structures of private images under $|M|>4$, which indicates that only reducing $|M|$ may not effectively improve the security of InstaHide. From Fig.~\ref{fig-different-epsilon} we observe \scheme\ can barely restore distinguishable visual features from encryptions generated from $\epsilon>0.4$, therefore reducing $|M|$ meanwhile increasing $\epsilon$ could be used to facilitate the security of InstaHide. In real-world applications, before releasing an encryption dataset, the data provider can attack this dataset with \scheme\ and accordingly adjust the parameters $|M|$ and $\epsilon$ to better protect the private images.

\noindent\textbf{Attack Performance under different types of public images.}
In the InstaHide Challenge dataset~\cite{instachallenge}, the authors only mix  public images with more than 40 key points (detected via SIFT~\cite{lowe2004sift}). We hence investigate the impact of different types of public images on the performance of \scheme\ and \cite{carlini2020attack}. 
%
% Both STL10 and CELEBA are used as the training and testing datasets. 
We fix $|M|_p=|M|_t=30$, $\epsilon_p=\epsilon_t=0.1$, and use public images with $[0, 10]$ key points (type 1), $[20, 30]$ key points (type 2) and $[40, 50]$ key points (type 3) to generate different encryption sets. Besides, we use Gaussian noises, whose mean and standard deviation equal to those of ImageNet, to generate random public images (type 4) and the corresponding encryptions.
% Fig.~\ref{fig-public} gives an example of mixing different types of public images with a same private image. We see that generally, flat public images can not effectively hide the information of private images.
%
Fig.~\ref{subfig-stl10-noise} and~\ref{subfig-celeba-noise} show the performance comparison between \scheme\ and~\cite{carlini2020attack} based on encryptions generated from different types of public images. Fig.~\ref{fig-different-noise} shows some restored images. 
% One observation from Fig.~\ref{subfig-stl10-noise} and~\ref{subfig-celeba-noise} is that both \scheme\ and~\cite{carlini2020attack} achieves better performance on datasets generated from type 2 public images than on datasets generated from type 1 public images. This counterintuitive result is mainly caused by color shift. When mixed with flat public images (type 1), the color profile, instead of the salient structures, of private images are severely corrupted. Since both \cite{carlini2020attack} and \scheme\ take mixed public pixels as Gaussian noise, and the distribution of type 2 pixels is more similar to Gaussian distribution than type 1, the quality of images restored from type 2 is better than the quality of images restored from type 1.
% Besides, the distribution of flat images is relatively difficult to estimate, leading to color shift in the restored images.
%
We observe that the performance of~\cite{carlini2020attack} greatly degrades when restoring private images based on type 3 public images, since type 3 images can severely corrupt the salient structure of the private images, leading to less information that can be used by ~\cite{carlini2020attack}. While such public images cause little degradation to \scheme, because different types of public images can barely change the distribution of noise components.
% and \scheme\ can learn this distribution and effectively remove it. 
In summary, when restoring private images from encryptions generated by InstaHide with data augmentation, public images with complicated patterns can degrade the performance of \cite{carlini2020attack} whereas causing little impact to \scheme.


% \begin{figure*}[t]
% \centering
% \includegraphics[width=.9\textwidth]{pic/differentNoise.pdf}
% \caption{Comparison of images restored from datasets mixed with different public images. For each block, the first row shows images restored by our scheme, and the second row shows images restored by \cite{carlini2020attack}}.
% \label{fig-different-noise}
% \end{figure*}

\begin{figure*}[t]
    \begin{subfigure}[b]{.25\textwidth}
            \includegraphics[width=0.95\textwidth]{pic/defenseM.pdf}
            \vspace{-2mm}
            \caption{Overall Performance}
            \label{fig-defenseM}
    \end{subfigure}%
    ~
    \begin{subfigure}[b]{.25\textwidth}
            \includegraphics[width=0.95\textwidth]{pic/stl10_noise.pdf}
            \vspace{-2mm}
            \caption{STL10}
            \label{subfig-stl10-noise}
    \end{subfigure}%
    ~
    \begin{subfigure}[b]{.25\textwidth}
            \centering
            \includegraphics[width=0.95\textwidth]{pic/celeba_noise.pdf}
            \vspace{-2mm}
            \caption{CELEBA}
            \label{subfig-celeba-noise}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{.2\textwidth}
            \includegraphics[width=0.95\textwidth]{pic/differentNoise.pdf}
            \vspace{-2mm}
            \caption{Examples}
            \label{fig-different-noise}
    \end{subfigure}%
\vspace{-4mm}
\caption{(a) shows the impact of reducing $|M|$ on the performance of the possible attacks; (b)-(c) show the SSIM \textit{w.r.t.} different types of public images; (d) shows the comparison of images restored by \scheme\ (first row) and \cite{carlini2020attack} (second row)  \textit{w.r.t.} different types of public images.}
\vspace{-4mm}
\end{figure*}


\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{pic/defenseMexp.pdf}
\vspace{-4mm}
\caption{Examples of images restored  by \scheme\ (first row) and \cite{carlini2020attack} (second row)  \textit{w.r.t.} reduced $|M|$.}
\label{fig-defenseM-exp}
\vspace{-4mm}
\end{figure}

==> tex/sec-overview.tex <==
\section{Attack Overview}

In this paper, we consider a data owner who utilizes InstaHide to protect the private image set $\mathcal{X}$ and publishes a training encryption set $\mathcal{M}$ as well as the corresponding label set $\mathcal{Y}_{\mathcal{M}}$. We assume that the $(\mathcal{M}, \mathcal{Y}_{\mathcal{M}})$ is accessible to the attacker since \cite{huang2020instahide} claims that a data owner can directly send the encryptions and labels to another party for training desired models. 
%
We assume that the published data is accessible to the data owner's collaborator since the authors of InstaHide~\cite{huang2020instahide} claim that a data owner can directly send the encryptions and labels to another party for training desired models. 
%
This paper focuses on the situation that the collaborator is the attacker. Specifically, the attacker aims to restore the data owner's private images $\mathcal{X}$ based on the published encryptions $\mathcal{M}$ and labels $\mathcal{Y}_{\mathcal{M}}$. 
%
In addition, the attacker may know the public image set $\mathcal{P}$ that is used for generating $\mathcal{M}$ in InstaHide (see Eq.~\ref{eq-instahide}) as it is public information.
Therefore, the attacker's goal can be formalized as:
\begin{equation}\label{eq-attack}
  \tilde{\mathcal{X}} = \mathcal{A}(\mathcal{M}, \mathcal{Y}_{\mathcal{M}}, \mathcal{P})
\end{equation}
where $\tilde{\mathcal{X}}$ is the inferred image set and $\mathcal{A}$ is the attack method executed by the adversary.


%we consider the semi-honest attack model~\cite{mohassel2017secureml} that the adversary only tries to infer private data based on known information instead of actively corrupting the training process. 
%Since InstaHide tries to protect the private images by generating a set of indistinguishable training encryptions $\mathcal{M}$, we assume that the adversary has $\mathcal{M}$ and the corresponding label set $\mathcal{Y}_{\mathcal{M}}$, and tries to restore the private image set $\mathcal{X}$. 

%This assumption is feasible because of two reasons: 
%first, some white-box attacks~\cite{zhu2020deep, zhao2020idlg} can precisely restore the input images based on model gradients, i.e. the encryption set $\mathcal{M}$ can be recovered by adversarial participants in the collaborative learning with high probabilities; 
%second, the authors of InstaHide~\cite{huang2020instahide} claim that some computationally limited participants can directly send their encryption sets to the central server for model training, but this server can be corrupted by a malicious adversary, or we can assume this server is an adversary. 
%Besides, since the one-hot labels $\mathcal{Y}_{\mathcal{M}}$ are not private~\cite{huang2020instahide}, from which the adversary can obtain the exact coefficients $\lambda^{(i)}_1$ and $\lambda^{(i)}_2$ for each encryption $m_i$.
%%%wyc: the above sentence could be mentioned in another place

%Consequently, the adversary aims to restore the private images $\mathcal{X}$ based on the training encryptions $\mathcal{M}$ and the corresponding labels $\mathcal{Y}_{\mathcal{M}}$:
%\begin{equation}\label{eq-attack}
%  \tilde{\mathcal{X}} = \mathcal{A}(\mathcal{M}, \mathcal{Y}_{\mathcal{M}}).
%\end{equation}

\subsection{Main Attacking Steps}
We now give an overview of the proposed attack method, as shown in Fig.~\ref{fig-overview}, which consists of three steps: absolute pre-processing, encryptions clustering and image restoring. 

\vspace{0.5mm}\noindent
\textbf{Absolute pre-processing}. In this step, we conduct $abs(m_i)$, for each encryption $m_i \in \mathcal{M}$, to preserve only the absolute pixel values. 
% \textcolor{blue}{(please add an explanation of why absolute value works here).}
This is consistent with~\cite{carlini2020attack}, since a pixel $p\in[-1, 1]$ consists of a sign and an absolute value. While the $\sigma$ mask renders the original signs to useless noise, yet failing to change the absolute pixel values. 
And the structures of the mixup image before encrypted by $\sigma$ are efficiently preserved by $abs(m_i)$ (Fig.~\ref{fig-mixegg}), which can be utilized by the subsequent  algorithms.
Note that we abuse the notation $m_i$ to refer to $abs(m_i)$ henceforth since the $abs$ operation is an indispensable step before the following restoration phases.

\vspace{0.5mm}\noindent
\textbf{Encryptions clustering}. Before restoring a private image ${x}_i$, we need to find a candidate set of encryptions $M$ from $\mathcal{M}$ containing the information of $x_i$.
We call the encryption set $M$ containing the same private image by \textit{homogeneous encryption set}.
%we need to find a candidate set of encryptions $M=\{m_{i,l}, l\in(0,\cdots,a)\}$ containing the information of $\hat{x}_i$ from $\mathcal{M}$ (we denote $m_{i}$ by $m_{i,0}$ and call the encryptions containing a same private image the \textit{homogeneous encryptions}). 
\cite{carlini2020attack} proposes to compute the similarity score between each pair of encryptions in $\mathcal{M}$ using a ResNet-28 model, and then cluster $\mathcal{M}$ such that encryptions in the same cluster contain the same private image.
%then clusters all the encryptions to find all the homogeneous encryption sets based on the similarity scores.
However, this method performs poorly against the proposed data generation method in Section~\ref{subsec-datageneration}, since the accuracy of ResNet-28 is severely degraded by useless periphery pixels produced by data augmentation. 
%
To attack InstaHide with data augmentation, we design a new comparative network in Section~\ref{subsec-com-nn} to compute the similarity between encryption pairs based on multi-resolution information of the encryptions, which achieves far better performance than \cite{carlini2020attack}. 
%The structure of the comparative network is shown in Fig.~\ref{fig-sim}.

\vspace{0.5mm}\noindent
\textbf{Image restoring}. After obtaining a homogeneous encryption set $M$, we present a fusion-denoising network (FDN) in Section~\ref{subsec-fdn} to restore the target image ${x}_i$. 
%%%wyc: not sure if this is necessary here
%We analyze the pixel variations of the private images caused by InstaHide and step 1, and find that in different encryptions, the corruption levels of a same private image are different. We then propose a re-weighting method to reduce the weight of the severely corrupted encryptions.
%   and focus on restoring the private image from the least corrupted encryption. 
The rationale behind FDN is that, although the visual features of private images are severely and non-linearly corrupted by the noise component introduced by InstaHide, the noise distributions contained in different encryptions are similar, and can be learned and accordingly removed by a  neural network. 
%After multiple trials, we design a fusion-denoising network (\scheme) which can learn such distributions from multiple homogeneous encryptions and hence restore the private images with high quality.
%The framework of \scheme\ is shown in Fig.~\ref{fig-fd}.
In particular, \scheme\ does not need an additional coloring phase employed in~\cite{carlini2020attack} because it can restore both the pixel intensities and signs of the target private images with high accuracy. 
%We give more details about the proposed attack in Sec.~\ref{sec-attack-detail}.


\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{pic/overview.pdf}
\vspace{-4mm}
\caption{Overview of the proposed attack.}
\label{fig-overview}
\vspace{-4mm}
\end{figure}

==> tex/sec-rebuttal.tex <==
\twocolumn

% \centerline{\textbf{\Large Rebuttal to Reviewers' Comments}}
% \vspace{10mm}

\noindent We thank the reviewers for their constructive suggestions. 
%%%wyc
In what follows, we provide a detailed response to each reviewer's comments, where RiQj denotes the response to Reviewer i's comments Qj.
%%%wyc: (comment out) We add more experiments on larger $\epsilon_p$s ({\color{red}R1}), different $\lambda$s and types of data augmentations ({\color{red}R4}), generalization of \scheme\ on different $\epsilon_p$s ({\color{red}R5}). We add more clarifications and explanations to address reviewers' concerns. 
%
% We believe the suggestions helped us to improve our submission. 
%%%wyc: (comment out) We hope that the reviewers have the chance to read our rebuttal and revise their scores.
%
For better readability, we call the InstaHide paper [HSL+] and Carlini et al.'s attack [CGD+].
% hereafter.







%\noindent{\color{red}R1}.
\noindent
{\color{blue}R1Q1}. In [HSL+], the authors suggest $k$ should be set up to 6 because the classifier trained with $k=6$ already suffers $10\%$ accuracy degradation. For our scheme, if changing $k$ from 4 to 6, the attack performance also suffers about 6\% degradation \textit{w.r.t.} SSIM as we use the same model to infer encryptions in different settings. 
%(a) we would like to note that in the experiments of [HSL+], the classifier trained with $k=6$ suffers $10\%$ accuracy degradation, which is the reason why the authors of [HSL+] recommend $k$ should be set up to 6. (b) we admit that when changing $k$ from 4 to 6, our scheme suffers up to SSIM $6\%$ degradation, because we use the same trained network to infer encryptions generated from different settings. 
However, even using $k=6$, \scheme\ still performs  $43\%$ better than CA. %We will add more clarifications in the paper.

\noindent{\color{blue}R1Q2}. As advised, we have added a new experiment, in which we fix $\mathcal{X}=\text{CIFAR10}$, $|M|=30$, and use an FDN trained with $\epsilon_t=0.3$ to attack the encryption sets generated with larger $\epsilon_p\in\{0.6, 0.7, 0.8, 0.9, 1\}$, the corresponding SSIMs are \{0.53,	0.51,	0.48,	0.45, 0.44\}. From Fig.~\ref{fig-rebuttal}a, we observe that the restored image quality degrades as $\epsilon_p$ increases.
% , which is because after the filtering step, less than 5 encryptions are retained as the input of \scheme.
However, 
% we would like to note that our main contribution is to issue a privacy alert to the possible variations of InstaHide.  
we further test the classification accuracies of a ResNet18 based on InstaHide with these $\epsilon_p$s, the results are $\{83.28\%,	81.51\%,	79.84\%,	78.36\%,	77.72\%
\}$, indicating a privacy-accuracy trade-off in larger $\epsilon_p$.

\noindent{\color{blue}R1Q3}. The filtering model is a binary classifier, with an $84\%$ accuracy tested on an image-pair dataset generated from ImageNet. We will report its performance in the paper.
% , which is used to infer whether the $\epsilon$'s of the input image pairs are less than a threshold. 
% We train the filtering model based on 





\noindent %{\color{red}R2}.
{\color{blue}R2Q1}. We would like to note that the variance can reflect the corruptness level of an encryption, and the variance-based factor can help better retain the information in the least corrupted ones.
We further train a network with only the $1/\lambda_1$ rescaling step, but obtained a $12\%$ SSIM degradation, which validates the effectiveness of the proposed re-weighting method.

% the re-weighting phase consists of two steps: first rescale all encryptions by the corresponding $\frac{1}{\lambda_1}$'s to recover the original   pixel intensity, then rescale the encryptions by a variance-based factor. As discussed in the paper, we need to focus on the encryption with the least corruptness level to obtain the best reconstruction performance, while  


\noindent{\color{blue}R2Q2}. 
%we would like to thank the reviewer for pointing out this issue. 
For an input set $\{x_1,\cdots,x_n\}$, we first feed them into the re-weighting, relaxing and CovBlock components one-by-one, and obtain a set of features $\{f(x_1),\cdots,f(x_n)\}$. These features will be merged into one feature $f(X)$ by the fusion component and fed into the denoising model.
% Because the fusion phase can merge any number of inputs into one image for the following processing, \scheme\ can accept a variable number of encryptions as the input. 
When $n\leq 10$, we recommend the choose-max fusion, otherwise the average fusion. We will add more explanations in the paper.

\noindent %{\color{red}R3}.
{\color{blue}R3Q1}. There are two main reasons. One is that the SSIM in Table~\ref{tab-ablation} is obtained by averaging the SSIM's of all test images, while the images in Table~\ref{tab-ablation} are randomly selected and may not correspond to the average values.
% for demonstrating the effects of different branches, which %%%wyc: what is the following sentence for?
The other is that SSIM considers luminance, contrast and structure simultaneously. The image in the no re-weighting branch has worse luminance and contrast but a better structure, which may cause the impression that it has better quality but lower SSIM. 
We will add more samples to Table~\ref{tab-ablation} for better justification.

%%%wyc: so the reviewer's comment is wrong?
\noindent{\color{blue}R3Q2}. 
%We thank the reviewer for pointing out this issue. 
We will carefully check the format of our submission. 




% \begin{wrapfigure}{r}{0.6\columnwidth}
% \centering
% \vspace{-2mm}
% \includegraphics[width=.7\columnwidth]{pic/rebuttalPic.pdf}
% \vspace{-3mm}
% \caption{New experimental results.}
% \label{fig-rebuttal}
% \vspace{-2mm}
% \end{wrapfigure}




\noindent %{\color{red}R4}.
{\color{blue}R4Q1}. Our scheme does not rely on any prior assumptions about data augmentation. In Preliminary, we classify data augmentation into geometric and non-geometric methods. 
%
In fact, the effects of non-geometric transformations can be covered by InstaHide because they are not used to eliminate the visual features. Thus, if \scheme\ works on InstaHide, then it can also work on non-geometric transformations. 

\begin{figure}[t]
\centering
% include first image
\includegraphics[width=.7\columnwidth]{pic/rebuttalPic.pdf}
%   \vspace{-2mm}
\vspace{-3mm}
\caption{New experimental results.}
%\vspace{-0.5cm}
\label{fig-rebuttal}
\vspace{-8mm}
\end{figure}

\noindent{\color{blue}R4Q2 \& R4Q3}. We have added new experiments \textit{w.r.t.} unknown augmentations to justify the generalization of our scheme. We first fix $\mathcal{X}=\text{CELEBA}$, $|M|=30$, 
%
then generate three InstaHide-encrypted datasets by applying \textbf{geometric} methods (random crop, perspective, rotation and affine with $\epsilon<0.5$), 
%
\textbf{non-geometric} methods (ColorJitter, GaussianBlur, Random Posterize and AdjustSharpness) and \textbf{mixed} methods, respectively. 
%
We use an \scheme\ trained with $\epsilon_p=0.3$ to attack them, and show the results in Fig.~\ref{fig-rebuttal}b.
We see that our scheme can successfully recover the private images pre-processed by unknown transformations with only a little color shift. We will add these new experiments in the paper.% which validate the generalization and effectiveness of our method.

\noindent{\color{blue}R4Q4}. %We conducted some preliminary comparison between SSIM $\ell_1$ and $\ell_2$ and in Table~\ref{tab-ablation}.
(a) We would like to refer the reviewer to Tab.~\ref{tab-ablation}, where we compare the effect of SSIM  with $\ell_1$ and $\ell_2$. 
(b) 
% Previous studies demonstrate that SSIM corresponds better to  human eyes. 
We give the SSIMs and $\ell_1$s in Fig.~\ref{fig-rebuttal}b. From left to right, we observe a degradation of image qualities, whereas the $\ell_1$ losses decrease and fail to correspond to the observation, because $\ell_1$ loss only examines luminance instead of structures. 
(c) To justify the selection of $\lambda$, we have added new experiments with $\lambda\in\{0.1, 0.3, 0.5, \textbf{0.7}, 0.9\}$ with the other parameters same as in \textbf{A2}. The resulting SSIMs are $\{0.59, 0.61, 0.62, \textbf{0.64}, 0.61\}$.

% \noindent\textbf{Why use SSIM instead of $\ell_1$ and $\ell_2$ (R4 Q4, R5 Q7)}. 
% Previous studies demonstrate that SSIM corresponds better to  human eyes. To justify, we give the SSIMs and $\ell_1$ losses in Fig.~\ref{fig-rebuttal}b. From left to right, we observe a degradation of image qualities, therefore we expect a decrease in SSIM and an increase in $\ell_1$. But the $\ell_1$ fails to correspond to the expectation. Because SSIM can examine luminance, contrast and structure while $\ell_1$ can only examine luminance.
% % , indicating that $\ell_1$ is not applicable to our task.

\noindent{\color{blue}R4D1}.
We note that [HSL+] has many follow-up studies since published in 2020. We demonstrate that the possible variations of InstaHide that can not be attacked by [CGD+] still suffer privacy risks. Importantly, there are substantial differences between our registration-fusion-denoising method and the optimization-based method in [CGD+].
%(a) we would like to mention that [HSL+], which claims that InstaHide can simultaneously protect the image privacy and improve the model performance, is pubished on ICML'20 and has 28 follow-up studies on Google Scholar, which may reflect its impact on the community.  (b)  [CGD+] demonstrate that private images can be reconstructed from the InstaHide Challenge dataset, which is ad-hoc and challenged by the authors of [HSL+] that it can not be used to attack the real-world variations of InstaHide, i.e., decreasing the mixup times of a private image, or incorporating geometrically transformations before mixup (see the instruction section). 
%We would like to highlight the contribution that our work demonstrates that the possible variations of InstaHide that can not be attacked by [CGD+] still suffer privacy risks. There are substantial differences between our registration-fusion-denoising method and the optimization-based method in [CGD+].

\noindent{\color{blue}R4D2}. 
%(a) we would like to thank the reviewer for this suggestion and note that the datasets used in [HSL+] are MNIST, CIFAR10 and CIFAR100. (b) as advised, 
As suggested, we have added an experiment on 10 randomly selected classes from the higher resolution ImageNet ($64\times 64$) with different $\epsilon$, and observed clearer differences in the results. We will report them in our paper.

\noindent% {\color{red}R5}.
{\color{blue}R5Q1 \& R5Q2}. $C$ consists of the coefficients of $\lambda_1$s and $\lambda_2$s, which can be inferred from the one-hot labels. For example, suppose there are four classes in a task. $x_1$ is of class 1 and $x_2$ is of class 3. Then the mix $m=\lambda_1 x_1+\lambda_2 x_2$ yields a label $y_m=[0.4\; 0\; 0.2\; 0]$, from which we infer $\lambda_1=0.4$.

\noindent{\color{blue}R5Q3}. By the central limit theory, if we view $\lambda_1 p^{{\hat x}_i}+p^\delta$ as a random variable $X_i$, then its mean $\Bar{X}_i$ follows a normal distribution.  \scheme\ can learn the relation between $\Bar{X}_i$ and $p^{{\hat x}_i}$, then accordingly infer the signs of $p^{{\hat x}_i}$.
% based on $\Bar{X}_i$.

\noindent{\color{blue}R5Q4 \& R5Q5}. 
% We first generate a large encryption-pair dataset from ImageNet, with homogeneous pairs labeled 1 and non-homogeneous pairs labeled 0, then feed each pair into the comparative network for training. 
The comparative network is a binary classifier. By testing accuracy, we indicate that for $92\%$ testing encryption pairs, the network can correctly determine whether the input pairs are homogeneous or not.
And the similarity score is the output of class 1 from the comparative network. We will provide more training settings in the Appendix.

\noindent{\color{blue}R5Q6}. We provided some examples of comparing image relaxing and convolutions in Fig. 3a and Table 2. 
% Due to space limitation, we put the ablation study, which compares the effects of image relaxing and convolutions in the appendix. 
% We will add more clarifications in the paper. 
%Fig.~\ref{fig-imgrelax}, which shows the results corresponding to our description. We further refer the reviewer to the ablation study (Tab.~\ref{tab-ablation}), which compares the effects of image relaxing (the original network) and convolutions (the no relaxing branch).

% \noindent{\color{blue}A7}. Previous studies have demonstrated that SSIM corresponds better to the human visual system than the $\ell_1$ and $\ell_2$ losses, because SSIM can simultaneously examine luminance, contrast and structure while $\ell_1$ and $\ell_2$ can only examine luminance. We would like to refer the reviewer to Fig. 2 in \textit{Image quality assessment: from error visibility to structural similarity} (2004) for more details.

\noindent{\color{blue}R5Q7}. We select SSIM because it corresponds better to human eyes. Please refer to R4Q4 (b) for an example.

\noindent{\color{blue}R5Q8}. For better justification, we have added an experiment with fixed $\mathcal{X}=\text{CIFAR10}$, $|M|=30$, and use \scheme s with different $\epsilon_t$ to attack the same encryption set with $\epsilon_p=0.3$. The results in Fig.~\ref{fig-rebuttal}c show that the \scheme\ trained with smaller $\epsilon_t$ can recover more details. We will check our claims and make sure that they are properly justified by experiments.





















==> tex/sec-related.tex <==
\section{Related Work}
\textbf{Image Registration and Fusion.} Image fusion is mainly used to integrate the complementary features of multiple images into one informative image~\cite{zhang2020ifcnn}. Before a successful fusion, the images capturing the same scene but in different perspectives should be geometrically aligned, which is known as \textit{image registration}. The traditional registration studies, including area-based methods and feature-based methods, mainly focus on extracting and aligning salient structures, such as edges and boundaries~\cite{ma2019infrared}. However, these methods are not useful if the image structures are severely corrupted.
% Traditional registration methods can be categorized into area-based methods and feature-based methods~\cite{zitova2003imgreg,ma2019infrared}. Area-based methods typically align two images based on their intensity values, which are obviously not applicable to InstaHide, since the original pixels of the target image in one encryption are randomly and severely corrupted. Feature-based methods first extract feature information (such as gradient histograms, feature points and edge maps) from two images and then estimate an optimal transformation. 
The \textit{image fusion} algorithms can be divided into three categories~\cite{ma2019infrared}: the spatial-domain fusion, such as extracting image features based on boundaries~\cite{zhang2017boundary}; the transform-domain fusion, such as multi-scale transform and sparse representation based image fusion~\cite{liu2015transform}; and the neural network based methods~\cite{zhang2020ifcnn}. Most fusion studies~\cite{zhang2017boundary, liu2015transform, zhang2020ifcnn} focus on fusing pre-registered images with the original pixels, but few of them considers the impact of image noise, especially when the input images are severely corrupted.

\vspace{0.5mm}\noindent\textbf{Image Denoising.}
Deep learning is widely used in image denoising tasks. REDNet~\cite{mao2016rednet} uses an encoder-decoder structure with skip connections to accelerate network convergence. RDN~\cite{zhang2020rdn} employs dense convolutional layers with residual connections to fully utilize the hierarchical features for image denoising. RNAN~\cite{zhang2019rnan} enhances the network representation capacity by attention mechanisms, which can learn long-range  dependencies in image features and performs better in restoring details from heavily corrupted images.
% In the proposed scheme, we adopt RNAN as the denoising component of the \scheme.
Besides, a few studies consider jointly image fusion and denoising~\cite{li2018joint, liu2020infrared, mei2019simultaneous} with the assumption that the input images are pre-registered and slightly corrupted by Gaussian  noises. 
% To the best of our knowledge, this is the first study exploiting joint image registration, fusion and denoising based on severely corrupted images with barely distinguishable salient structures.

\vspace{0.5mm}\noindent\textbf{Mixup.}
Mixup is proposed in~\cite{zhang2017mixup} as a regularization method for neural network training.
% , which trains neural networks based on mixup datasets generated by mixing two training images and the corresponding labels.
%Some studies employ Mixup to increase the robustness and generalization of neural networks. For example, \cite{beckham2019adversarial} uses Mixup to combine different representations learned by auto-encoders for synthesizing realistic images. \cite{berthelot2019mixmatch} proposes to improve the accuracy of semi-supervised learning using Mixup, i.e., generating a new training dataset by mixing the labeled and unlabeled images.
Since Mixup can obfuscate the visual features of images, some recent studies
~\cite{fu2019mixup, raynal2020image} employ it to pre-process the raw training data for privacy preserving.
%
However, the attack proposed in~\cite{huang2020instahide} demonstrates that if one private image is mixed multiple times, then it can be simply restored by averaging those mixup images containing it. Accordingly, \cite{huang2020instahide} propose InstaHide to enhance the security of Mixup.
% which generates one encryption image by first mixing multiple public images with two private images then randomly flipping the signs of the mixup images.
% The authors of~\cite{huang2020instahide} further released an InstaHide Challenge dataset to encourage effective attacks on InstaHide.
%
But~\cite{carlini2020attack} proposes an attack that can successfully restore distinguishable images from the InstaHide Challenge dataset~\cite{instachallenge} by minimizing the norm of the noise component corresponding to the public images.
Nevertheless, \cite{carlini2020attack} is specifically designed for the original InstaHide scheme, which is hardly applicable to other modified InstaHide schemes.

% In this paper, we consider a more complicated and real setting, i.e., restoring images from the encryption datasets which are generated by first transforming the private images via data augmentation then applying InstaHide on these transformed images. The experiments demonstrate that both the generalization and effectiveness of the proposed scheme are superior \cite{carlini2020attack}.

==> tex/sec-reviews.tex <==
\twocolumn

\section*{Reviewer 1 (Borderline Accept)}
Questions to answer:
\begin{enumerate}
    \item The performance of the proposed method degrades as $k$ (the number of confounding images in each encryption) increases. This is a significant limitation of the proposed approach compared to (Carlini et al. 2020) whose performance increases as $k$ increases. Additional exploration of this limitation beyond the analysis for $k$=4 and 6 in the appendix is warranted.
    \item The classification accuracy of models trained with instaHide does not change when the eps-augmentation level is increased from 0 to 0.5 (See figure 7 of the Appendix). This suggest that instaHide can support a much higher level of eps-augmentation, yet the performance of the proposed attack method degrades significantly when the eps-augmentation level is increased from 0 to 0.5 (See Table 1). Is it the case that the proposed attack method can be thwarted by simply increasing the eps-augmentation level? Additional experiments are required to answer this question.
    \item The performance of the pre-filtering network is not reported.
\end{enumerate}

\section*{Reviewer 2 (Weak Accept)}
Questions to answer:
\begin{enumerate}
    \item The motivation to re-weight the encryptions based on their variances is unclear. Why not use a factor directly based on the coefficients $\lambda_1$?
   \item The multiple-channel fusion architecture in Fig. 6 is unclear. There are no explanations on why the fusion model can accept a variable number of encryptions as the input and whether to use choose-max rule or average rule.
\end{enumerate}

\section*{Reviewer 3 (Accept)}
Questions to answer:
\begin{enumerate}
    \item From the table 2, the ssim of No Img. Relaxing is better than that of No Reweighting. But the image quality of No Img. Relaxing is worse. What the reason is it.
    \item Following the the submission in violation of the AAAI format, the number and caption for your table must apper under the table.
\end{enumerate}


\section*{Reviewer 4 (Borderline Reject)}
Questions to answer:
\begin{enumerate}
    \item The work considers a very specific type of augment. I understand this work is built upon the work by Carlini et al. but what happens if people use other types of data augmentation? Doesn't this works assume that at least data augmentation mechanism should be known a priori? This seems to me a very strong assumption.
    \item What happens if several types of very different augmentation methods are used?
    \item In case of the above (unkonw augmentation type or several types of augmentation), is it possible to train the fusion network such that it performs decently.
    \item No ablative experiments are provided to demonstrate that SSIM is indeed effective. I think experiments should be performed using L1 and L2 metrics as well as various values for $\lambda$ to study the effectiveness of SSIM in this application.
\end{enumerate}

Detailed Feedback for the Authors:
\begin{enumerate}
    \item An area that affects my rating is that the algorithm is too focused on a very recently developed method which is not clear to me that will become a widespread method. Hence, I am a concerned that the paper is addressing a problem that does not have enough practical importance. On the other hand, the novelty of this work seem to be incremental based on improving an existing work. As a result, I am not sure this work is of the caliber of a conference like AAAI.
    \item The datasets used for experiments are relatively simple. I think it is important to test the method on more realistic datasets such as ImageNet. In particular, you can see that differences in Figure 4 are not easily observable. My guess is that using larger images will boost the differences and clarifies the effectiveness of the proposed method further.
\end{enumerate}

\section*{Reviewer 5 (Borderline Accept)}
Questions to answer:
\begin{enumerate}
    \item In p.3 left column before (2), how do one know $C$ while solving $A$?
    \item In p.3 right column, how does one infer $\lambda_1$ from the one-hot labels?
    \item  In p.3 right column, is there any intuitive reasons why neural network can roughly infer the signs of $\lambda_1 p^{{\hat x}_i}+p^\delta$?
    \item Regarding to Figure 2, please give more details on how to train neural networks so as to compare the similarity scores.
    \item  In p.4 right column, it is mentioned that "the testing accuracy of the proposed network can reach 92$\%$". What do you mean by testing accuracy? As the context around this sentence seam to refer to the computation of similarity score, and it is not clear if such ground truth is available and in what format.
    \item In p.5 left column, the authors try to compare the effects of image relaxing to CNNs by words. I would suggest the authors provide more evidences that can be objectively verified beyond merely description wordings that are difficult to verify.
    \item In experiment the authors mentioned of applying MSSIM with window size 8 to measure the similarity. Why the authors choose such metric? Does such metric align to previous works, as well as providing a fair comparison ground?
    \item In p.6 left column, the authors mention "The reason is that when trained on a dataset with smaller transformations, the FDN learns to restore more image details instead of focusing on registering image structures. Nevertheless, when tested on a specific $\epsilon_p$, different FDNs perform similarly, demonstrating the good generalization of FDN under different augmentation levels". Is such claim supported by verifiable experimental results? There are quite some other statements like this which lack of convincing experimental or theoretical support.
\end{enumerate}

























